CLOAK: A Framework For Development of Confidential Blockchain Smart Contracts

In recent years, as blockchain adoption has been expanding across a wide range of domains, e.g., digital asset, supply chain finance, etc., the confidentiality of smart contracts is now a fundamental demand for practical applications. However, while new privacy protection techniques keep coming out, how existing ones can best fit development settings is little studied. Suffering from limited architectural support in terms of programming interfaces, state-of-the-art solutions can hardly reach general developers. In this paper, we proposed the CLOAK framework for developing confidential smart contracts. The key capability of CLOAK is allowing developers to implement and deploy practical solutions to multi-party transaction (MPT) problems, i.e., transact with secret inputs and states owned by different parties by simply specifying it. To this end, CLOAK introduced a domain-specific annotation language for declaring privacy specifications and further automatically generating confidential smart contracts to be deployed with trusted execution environment (TEE) on blockchain. In our evaluation on both simple and real-world applications, developers managed to deploy business services on blockchain in a concise manner by only developing CLOAK smart contracts whose size is less than 30% of the deployed ones.

==> architecture.tex <==

\subsection{The overview of TEE-based privacy architecture}
In this section, we introduce the details of the TEE-based privacy architecture. Figure~\ref{fig:cloak-tee} shows overview of the architecture. $F$ means contract code that clearly expresses the business logic $f$ of VMPT. $P$ is a privacy policy, which expresses the privacy specification of VMPT, specifically what's the secret data and who are participants. $E$ is able to receive private data, run $F$, generate proof $p$ and deliver result. $V$ is a public verifier, which is responsible for verifying the legitimacy of the $S'$ with $p$ and update state. 

In following, we will introduce how to simultaneously achieve the security properties $P1\wedge P2\wedge P3$ of VMPT based on this architecture.


\begin{figure}[h]
  \includegraphics[width=8.5cm]{images/vp-arch.png}
  \caption{TEE-based verifiable privacy architecture}
  \label{fig:cloak-tee}
\end{figure}

\subsection{Privacy policy of VMPT}

To achieve $P1$, we should avoiding privacy leakage both in execution and in inputs parameter or return value. As executing $F$ in enclaves has already achieved execution privacy, we additionally need to specify privacy policy, $P$, to instruct $E$ enforce the privacy of input and output. The privacy specification of the MPC protocol will be limit by $P$ hash.

\subsection{Target function of VMPT}


To achieve $P2$, we could easily express the $f$ of VMPT by smart contracts, marked as target function $F$, and limit it by $F$ hash.

Although $F$ is expected to be expressed in a user-friendly way, it's never limited by blockchain supported contract language. We will further explain this in session~\ref{sec:tee-verifier}.

\subsection{TEE-based executor of VMPT}
To achieve $P3$, we first need basic run-time of $E$, then we will introduce how to construct the proof of MPT result that proves the bound of the typle, $(F, P, E)$.

\subsubsection{Enclave runtime}
$E$ is the core of the architecture, it consists of three modules, Privacy Interpreter Enclave (PIE), Key Management Enclave (KME) and Virtual Machine Enclave (VME). The participants of an VMPT seals their secret $x_i$, and transaction info, \eg function name and contract name, by $E$'s public key, sign the transaction, and send it to the $E$. Upon receiving the request, $E$ revealing the data and processes the transaction by PIE, PIE reads the transaction related $P$, $S$, and $F$ from the ledger, then, wait to receive secrets from all parties. After secrets are obtained and checked, PIE call VME to execute $F$. When the execution finished, PIE enforce $y_i$ private to $x_i$. It also encrypt new plaintext state according to $P$ to get $S'$, sends a transaction with $S'$ and proof to update the verifier's old state, $S$.

As $F$ is expressed by Solidity here, the VME of $E$ should hold Ethereum Virtual Machine (EVM) to run the compiled bytecode. We note that VME could be easy to expand to WASM, JVM, \etc. 

\subsubsection{Proof generation}\label{sec:proof-generation}

To achieve $P2$, we built a trust chain based on the \textit{Non-broken device assumption}. The assumption means the real TEE device has not been compromised. We note that this is an easy-to-reach assumption and adopted in lots of related works~\cite{matetic2018delegatee, Sinisa2019BITE}. Furthermore, we'd also propose practical ways to reduce the risk of broken assumption. This will be discussed in session~\ref{sec:tee-consensus}. Based on this assumption, we integrate three proofs to achieve the whole verifiablity.

\myparagraph{Device authenticity proof}
The trust of SGX device is based on a remote attestation report from Intel IAS. Thus, we first attest and publish the report of each SGX. 

\begin{lstlisting}[caption=Simplified attestation report of SGX from Intel IAS, label=listing:proofData][!htbp]
{
    "X-IASReport-Signature": <string>,  
    "reportData": {
        "isvEnclaveQuoteStatus": <string>,
        "isvEnclaveQuoteBody": <string> {
            "REPORTBODY": {
                "MRENCLAVE": <string>,
                "REPORTDATA": <string>
            }
        }
    }
}
\end{lstlisting}

\myparagraph{Trust runtime proof}
Based on real SGX devices, we also need to prove that the communication channel and code runtime is trusted. To defend the user from Man in the middle attack, two keys $E_{pk}$, \textit{encKey}, and $V_{pk}$, \textit{verKey}, will be bound in the IAS report. $E_{pk}$ is an encryption key, \eg RSA public key, with which users can make sure only the code in enclave available to private data. $V_{pk}$ is a verification key, \eg ECDSA public key, with which users can make sure the authenticity of results. Then, with a bound code hash, \textit{TEEMRs}, the in-mutable of executor runtime is also achieved.

\begin{lstlisting}[language=Solidity, caption=The registration data of SGX on-chain, label=listing:registerData][!htbp]
struct RegisterData {
    string verKey;
    string encKey;  
    string[] TEEMRs; 
    string IASReport;
}
\end{lstlisting}

List~\ref{listing:registerData} shows the data structure used by SGX to register itself on-chain before receiving users' private data. It would be verified by users to make sure device authenticity and executor trust.

\myparagraph{Result proof}
To prove that the result is the real result of the private contract with the expected $F$ and $P$. SGX sign the report with the hash of $F$, $P$, $S$ and $S'$ using the signing key corresponding to $V_{pk}$ of trusted runtime $E$. The report could be the verifiable MPC proof, $p$.


\subsection{On-chain contract verifier}\label{sec:tee-verifier}
To verify $p$ on-chain, \codename will deploy the predefined \texttt{CloakService} and verifier contract to blockchain first. These contracts wholly call $V$.

\subsubsection{TEE executor registration contract}
\texttt{CloakService} is deployed for registering the $E$'s runtime proof. It register IAS reports to make them in-mutable and available. verifier contract would call \textit{verify} to check the proof of VMPT.

\subsubsection{Transaction result verifier contract}
% With \texttt{CloakService}, \codename processes all annotated private function of smart contract and generate a corresponding on-chain contract for verification. 

The verifier contract will call \texttt{CloakService} to verify two conditions. First, the transaction's original sender matched one of the registered TEE with the specific SGX measurement in the pool. Second, the bound of $F$, $P$, $S$ is expected. If all these are satisfied, the verifier contract will update its contract state. An example of a verifier will be showed in session~\ref{sec:verifier-contract}.

\begin{lstlisting}[language=Solidity, caption=The generated service contract, label=listing:contracts]
contract CloakService {
  mapping<address => RegisterData> public devicesInfo;
	
	function registerWorker(
	    address workerId, 
	    RegisterData deviceInfo
	) public {
		// check deviceInfo, register a new TEE device 
	}

	function verify(
		uint256[] proof,
	    uint256 TEEMR,
	    uint256 codeHash, 
	    uint256 policyHash, 
	    uint256 functionHash,
	    uint256 oldStateHash,
	) public returns (bool) { 
		// check tx.origin, codeHash, policyHash
		return true;
	}
}
\end{lstlisting}

\subsection{Optimizations}

\subsubsection{Patch processing transactions as Layer-2}
As a state machine, a blockchain world state transforms according to old state and new transactions. We can batch process the transactions. The scalability of the \textit{VP-Arch} could be significantly higher than the main chain. \textit{VP-Arch} could periodically synchronize the state with the main chain or synchronize the state responding to the user request.


\subsubsection{Improve credibility through consensus}\label{sec:tee-consensus}
We apply a consensus between $E$ to reduce the risk of devices being compromised. Since all known SGX attacks require to access the device and cause limited loss~\cite{Zhang2020SurveyOA, Nilsson2020ASO}, SGX-based nodes are believed as None-Byzantine nodes in some degree, which makes \textit{VP-Arch} high scalable and trusted.


